On Solving Reachability in Grid Digraphs using a Psuedoseparator

The reachability problem asks to decide if there exists a path from one vertex to another in a digraph. In a grid digraph, the vertices are the points of a two-dimensional square grid, and an edge can occur between a vertex and its immediate horizontal and vertical neighbors only. Asano and Doerr (CCCG'11) presented the first simultaneous time-space bound for reachability in grid digraphs by solving the problem in polynomial time and $O(n^{1/2 + \epsilon})$ space. In 2018, the space complexity was improved to $\tilde{O}(n^{1/3})$ by Ashida and Nakagawa (SoCG'18). In this paper, we show that there exists a polynomial-time algorithm that uses $O(n^{1/4 + \epsilon})$ space to solve the reachability problem in a grid digraph containing $n$ vertices. We define and construct a new separator-like device called pseudoseparator to develop a divide-and-conquer algorithm. This algorithm works in a space-efficient manner to solve reachability.

==> tocspecial.tex <==
%% tocspecial.tex 2020-09-01  Version 0.22  ToC style file
%------------------------------------------------------------------
% Filename: tocspecial.cls
% 
% This documentclass is intended for typesetting articles for the
% 
% Theory of Computing.
% 
% See http://theoryofcomputing.org for further details.
%
% Version 0.1 Initial combination of banners from previous style files.
% Version 0.2 Addition of CCC banners. Clean up.
% Version 0.21 Addition of more CCC banners, up to 2023
% Version 0.22 Rename \boolean --> \aboolean to avoid clash with ifthen.
% ------------------------------------------------------------------
%
%% Special issue banners:

%% explanation: BC = 2012 BD = 2013 ... CA = 2020 CB = 2021 ...

\newcommand{\motwani}{Special issue in honor of Rajeev Motwani}
\newcommand{\aboolean}{Special issue: Analysis of Boolean Functions}
\newcommand{\approxrandomBC}{Special issue: APPROX-RANDOM 2012}
\newcommand{\approxrandomBD}{Special issue: APPROX-RANDOM 2013}
\newcommand{\approxrandomBE}{Special issue: APPROX-RANDOM 2014}
\newcommand{\approxrandomBF}{Special issue: APPROX-RANDOM 2015}
\newcommand{\approxrandomBG}{Special issue: APPROX-RANDOM 2016}
\newcommand{\randomBI}{Special issue: RANDOM 2018}
\newcommand{\approxrandomBJ}{Special issue: APPROX-RANDOM 2019}
\newcommand{\cccBF}{Special issue: CCC 2015}
\newcommand{\cccBG}{Special issue: CCC 2016}
\newcommand{\cccBH}{Special issue: CCC 2017}
\newcommand{\cccBI}{Special issue: CCC 2018}
\newcommand{\cccBJ}{Special issue: CCC 2019}
\newcommand{\cccCA}{Special issue: CCC 2020}
\newcommand{\cccCB}{Special issue: CCC 2021}
\newcommand{\cccCC}{Special issue: CCC 2022}
\newcommand{\cccCD}{Special issue: CCC 2023}

